Hierarchical Cross-Modal Agent for Robotics Vision-and-Language Navigation

Deep Learning has revolutionized our ability to solve complex problems such as Vision-and-Language Navigation (VLN). This task requires the agent to navigate to a goal purely based on visual sensory inputs given natural language instructions. However, prior works formulate the problem as a navigation graph with a discrete action space. In this work, we lift the agent off the navigation graph and propose a more complex VLN setting in continuous 3D reconstructed environments. Our proposed setting, Robo-VLN, more closely mimics the challenges of real world navigation. Robo-VLN tasks have longer trajectory lengths, continuous action spaces, and challenges such as obstacles. We provide a suite of baselines inspired by state-of-the-art works in discrete VLN and show that they are less effective at this task. We further propose that decomposing the task into specialized high- and low-level policies can more effectively tackle this task. With extensive experiments, we show that by using layered decision making, modularized training, and decoupling reasoning and imitation, our proposed Hierarchical Cross-Modal (HCM) agent outperforms existing baselines in all key metrics and sets a new benchmark for Robo-VLN.

==> tables/ablation2.tex <==
\begin{table*}[ht]
\scriptsize
\centering
\caption{\textbf{Ablation Study}: Comparison of }
\label{comprehensive}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{c*{15}{>{$}c<{$}}}
\toprule
& & \multicolumn{3}{c}{\textbf{Module}} \multicolumn{5}{c}{\textbf{Validation Seen}} &\multicolumn{5}{c}{\textbf{Validation Unseen}} \\ 
\cline{3-5}\cline{6-10}\cline{11-15} \\ 
& \# & \text{Vision} &\text{Hierarchy} &\text{RGB-D Early fusion} & \textbf{SR}\uparrow & \textbf{SPL}\uparrow & \textbf{NDTW}\uparrow & \textbf{TL}\uparrow & \textbf{NE}\downarrow & \textbf{SR}\uparrow & \textbf{SPL} & \textbf{NDTW}\uparrow & \textbf{TL}\uparrow & \textbf{NE}\downarrow\\
\midrule
& 1 & &\checkmark &  & 0.07 & 0.07& 0.14& 4.83 & 10.34 & 0.07& 0.07 & 0.14 & 10.20 & 4.81  \\
\textbf{SASRA} & 2 &\checkmark& & & 0.44& 0.37 & 0.31 & 14.87 & 8.21 & 0.40 & 0.34 & 0.29 &  15.32 & 8.64  \\
\textbf{Agent} & 2 &\checkmark& \checkmark& \checkmark & 0.39 &  0.35 & 0.29 & 13.88 & 9.13 & 0.34 & 0.31 & 0.28 & 12.85 & 8.78  \\
& 3 &\checkmark&\checkmark &\checkmark & 0.19 & & & & & & 0.204 & & &  \\
\midrule
\end{tabular}
}
\end{table*}
